Taxonomy of Machine Learning Safety: A Survey and Primer

The open-world deployment of Machine Learning (ML) algorithms in safety-critical applications such as autonomous vehicles needs to address a variety of ML vulnerabilities such as interpretability, verifiability, and performance limitations. Research explores different approaches to improve ML dependability by proposing new models and training techniques to reduce generalization error, achieve domain adaptation, and detect outlier examples and adversarial attacks. However, there is a missing connection between ongoing ML research and well-established safety principles. In this paper, we present a structured and comprehensive review of ML techniques to improve the dependability of ML algorithms in uncontrolled open-world settings. From this review, we propose the Taxonomy of ML Safety that maps state-of-the-art ML techniques to key engineering safety strategies. Our taxonomy of ML safety presents a safety-oriented categorization of ML techniques to provide guidance for improving dependability of the ML design and development. The proposed taxonomy can serve as a safety checklist to aid designers in improving coverage and diversity of safety strategies employed in any given ML system.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typset multiple affiliations (Christoph Sommer)

==> sections/2.1-extended-background.tex <==


% % >>> [domain shift] --> manually perturbed 
%                      --> seasonal change/locations changes 
% % - ImageNet-A and ImageNet-O: used different test source --> [domain shift]
% % - ImageNet-R:                [domain shift]
% % - ImageNet-C and ImageNet-P: [domain shift]
% - BDD-100k dataset \cite{yu2020bdd100k} covers diverse weather conditions (sunny/rainy/snowy) and different time of day (daytime/nighttime/dusk/dawn) to benchmark autonomous driving scenes. 
% % - ImageNet-9: 

% >>> [generalization error] --> 
% -            : used the same dataset
% ImageNet-v2: used the same collection pipeline --> [generalization error]


%% 1- Empirical Error:      generalization error on i.i.d test set
%% 2- Distributional Error: generalization error on (naturally shifted/perturbed test set)
%% 3- Adversarial Error:    generalization error on (adv. perturbed test set)


\vspace{-0.5em}
\section{ML Dependability}
\label{sec:error-types}

Dependability is the model's ability to minimize prediction risk on test samples. 
% Unlike code-based algorithms, the dependability of ML algorithms is bounded to the model's learning capacity and statistical assumptions under which the model is trained.
% Examples of these assumptions include the independent and identically distribution (i.i.d) relation of source and target domains. 
% % and the assumption for uniform distribution of data across all classes (i.e., class balance) \cite{domingos2012few,l2017machine}. % We don't discuss imbalanced datasets so this is removed.
% However, maintaining data distribution assumptions when deployed in the open-world is challenging and results in different types of prediction errors. 
In this section, we categorize model dependability into three different dimensions: generalization error (Sec. \ref{sec:generalization_error}), robustness against distributional shift (Sec. \ref{sec:distributional_shift}), and robustness against adversarial attacks (Sec. \ref{sec:adversarial_attack}).
% as a unified ``big picture'' to achieve dependable and robust ML models in open-world. 
Additionally, we review benchmark datasets commonly used for each type of model dependability.

\vspace{-0.5em}
\subsection{Generalization Error} \label{sec:generalization_error}
The first and foremost goal of machine learning is to minimize the \emph{generalization error}.
Given a hypothesis $h$ (e.g., a DNN with learned parameters), the generalization error (also know as the \emph{true error} and denoted as $R(h)$) is defined as the expected error of $h$ on the data distribution $\mathcal{D}$~\cite{mohri2018foundations}:
$
    R(h) = \text{Pr}_{(x,y) \sim \mathcal{D}}[h(x)\neq y] = \mathbb{E}_{(x,y) \sim \mathcal{D}}[\mathbbm{1}_{h(x)\neq y}],
$
where $(x,y)$ is a pair of data and label sampled from $\mathcal{D}$, and $\mathbbm{1}$ is the indicator function. 
The generalization error is not directly computable, since $\mathcal{D}$ is usually unknown. 
The \textit {de facto} practical solution is to learn $h$ by empirical risk minimization (ERM) on the training set $\mathbb{S}_{S}=\{(x_i,y_i)\}_{i=1}^{N_S}$ and estimate its generalization error by the \emph{empirical error} on the holdout test set $\mathbb{S}_{T}=\{(x_i,y_i)\}_{i=1}^{N_T}$. 
Formally, the empirical error $\hat{R}(h)$ is defined as the mean error on a finite set of data points $\mathbb{S} \sim \mathcal{D}^{m}$~\cite{mohri2018foundations}:
$
    \hat{R}(h) = \frac{1}{m} \sum_{i=1}^{m} \mathbbm{1}_{h(x_i)\neq y_i},
$
where $\mathbb{S} \sim \mathcal{D}^{m}$ means $\mathbb{S}=\{(x_i,y_i)\}_{i=1}^m \overset{i.i.d.}{\sim} \mathcal{D}$.
The training and test sets are all sampled from the same distribution $\mathcal{D}$ but are disjoint.
% Consider a model learned by empirical risk minimization (ERM) on training set $S=\{(x_i,y_i)\}_{i=1}^N$ i.i.d sampled from the underlying distribution $\mathcal{D}$.
% The model should not only fit $S$ by minimizing the empirical error $\mathcal{L}_\mathcal{S}(f)=\frac{1}{N}\sum_{x \in \mathcal{S}}~\mathcal{L}(x)$, but also have low generalization error on unseen data $\mathcal{L}_\mathcal{D}(f)=\mathbb{E}_{x \in \mathcal{D}} ~\mathcal{L}(x)$. 
% The generalization gap is defined as the difference between the model performance on training data and unseen data sampled from the same distribution, is a commonly used metric to evaluate model generalization ability.
% The \textit {de facto} method nowadays of probing generalization is to split the available dataset into two (or three) subsets: one for training, (one for validation), and the other for testing. The goodness of fit on the test set provides an approximation of generalization beyond training. 
Recent years have witnessed the successful application of this holdout evaluation methodology to monitoring the progress of many  ML fields, especially where large-scale labeled datasets are available. 
The generalization error can be affected by many factors, such as training set quality (e.g., imbalanced class distribution \cite{haixiang2017learning}, noisy labels \cite{bouguelia2018agreeing}), model capacity, and the training methods (e.g., using pre-training \cite{mahajan2018exploring}, regularization \cite{bansal2018can}, etc.)
% Multiple factors such as weak representation learning affect the model's generalization error which is common in open-world setups \cite{jakubovitz2019generalization}. % (e.g., model over-fitting or under-fitting on the training set)
% On the importance of generalizable representation learning, Zhang et al. \cite{Zhang2017generalization} pointed out the capacity of large DNNs is sufficient enough to memorize a small training set even in the case of random labels without any correlation between training labels and test labels. 
% On the other hand, the training set quality can greatly affect model generalization error as many assumptions such as uniform distribution of training data may not be easy to achieve in open and uncontrolled environments. 
% This is because of the large number of model parameters in the network that may exceed the number of data points in training sets, resulting in relatively small generalization error on their test set, but a high error rate on slight domain shifts within the same label space (i.e., hyper-parameter over-fitting). 
% However, representation learning gets more difficult when aiming for more complex tasks and using data with higher dimensionality. 


\paragraph{Benchmark Datasets:} 
Model generalization is commonly evaluated on a separate test set provided for the dataset.
However, recent research has found limitations of such evaluation strategy. 
For example, \citet{wang2020going} showed that the fixed ImageNet \cite{deng2009imagenet}  test set is not sufficient to reliably evaluate the generalization ability of state-of-the-art image classifiers, due to the insufficiency in representing the rich visual open-world.
% Other efforts have been made to collect new samples to improve test sets for image classification tasks. % as complements for the original ImageNet test set. 
\citet{tsipras2020imagenet} observed that noisy data collection pipeline can lead to a systematic misalignment between the training sets and the real-world tasks. % a brittleness that puts claims about human-level performance into context.



\vspace{-0.5em}
\subsection{Robustness against Distributional Shifts} 
\label{sec:distributional_shift}
When measuring generalization error, we assume the source training set $\mathbb{S}_S$ and the target test set $\mathbb{S}_T$ are from the same data distribution. 
However, this assumption is frequently violated in real world applications. In other words, we will have $p_S(x,y) \neq p_T(x,y)$ where $p_S(x,y)$ and $p_T(x,y)$ are the joint probability density distributions of data $x$ and label $y$ on the training and test distributions, respectively.
Such mismatch between training and test data distribution is known as \textit{dataset shift}~\cite{quinonero2009dataset} (also termed as \textit{distributional shift} or \textit{domain shift} in literature).
In this paragraph, we describe two most common distributional shifts and their benchmark datasets. 
\textit{Covariate shift} means that the training and test distributions of the input covariate $x$ are different (i.e., $p_S(x) \neq p_T(x)$), while the labeling function remains the same (i.e., $p_S(y|x) = p_T(y|x)$). 
Covariate shift may occur due to natural perturbations (e.g., weather and lighting changes), data changes over time (e.g., seasonal variations of data), and even more subtle digital corruptions on images (e.g., JPEG compression and low saturation). 
\textit{Label distribution shift} (also know as \textit{prior probability shift}) is the scenario when the marginal distributions of $y$ changes while the class-conditional distribution remains the same. Formally, it is defined as $p_S(y) \neq p_T(y), p_S(x|y) = p_T(x|y)$.  
Prior probability shift is typically concerned in applications where the label $y$ is the casual variable (e.g., pneumonia) for the observed feature $x$ (e.g., chest X-ray) \cite{lipton2018detecting}. For example, if we trained a pneumonia predictor using the chest X-ray data collected in summer (when $p(y)$ is low), we may still require it to be accurate on patients visiting in winter (when $p(y)$ is high).
A special case for label distributional shift is long-tailed recognition \cite{van2017devil}, where the training set is long-tail distributed (i.e., $p_S(y)$ follows a long-tailed distribution) while the test set is balanced (i.e., $p_T(y)$ roughly follows a uniform distribution).

% Domain shift (also known as distribution shift and dataset shift) describes variations in the target data distribution ($D_{target}$) in comparison to the source training distribution ($D_{train}$). 
% Distributional error is the misprediction of target samples due to inconsistency between source and target distributions and hence reduces the \textit{Operational Performance} compared to the test set (on $D_{test}$) performance.
% Specifically, distributional error reduces the operational performance compared to the training set performance (on $D_{test}$) by breaking the i.i.d assumption between source and target data. 
% In this regard, robust training techniques (e.g., transfer learning, domain generalization) are necessary elements in training ML models for open-world applications in which target samples are captured from uncontrolled and constantly changing environments (see Section \ref{sec:RT} for details).

% Common examples of domain shift include non-semantic distribution changes due to input perturbations (e.g., natural perturbations due to weather and lighting changes), data changes over time (e.g., seasonal variations of data), and even more substantial texture and breed variations. % geographic locations.
% In general, the problem of ``domain shift" is rooted in the fundamental contradiction between the enormous size and high dimensionality of natural image manifold, and the limited scale of affordable testing (i.e., human labeling, or verifying predicted labels, which is expensive and time consuming).
% Model comparison based on a limited number of samples assumes that they are \textit{sufficiently representative} of the whole population, an assumption that has been proven to be doubtful in computer vision tasks. 
% On studies to measure the distributional error, different work shows that using a fixed test set are insufficiently representative of the whole target distribution. 
% For instance, Recht et al. \cite{recht2018cifar,recht2019imagenet} found that a minute natural distribution shift leads to a large drop in accuracy for a broad range of image classifiers on both CIFAR-10~\cite{krizhevsky2009learning} and ImageNet. %  suggesting that the current test sets may be far from sufficient to represent hard natural images encountered in the real world. 


% Beyond generalization to reasonably foreseeable domain shifts, Out-of-Distribution (OOD) or outlier samples are referred to undesirable test-time samples with disjoint label space and high semantic discrepancy. 
Beyond the above reasonably foreseeable domain shifts, a model may also encounter out-of-distribution (OOD) test samples with semantic contents unseen in the training distribution. 
For example, for a classifier trained on hand-written digit images, a Roman character is an OOD test sample (while a printed digit is a test sample with domain gap).
\textit{OOD detection} \cite{hendrycks2016baseline} is the approach to detect such OOD samples, whose predictions will be rejected (see Section \ref{sec:ood-detection} for details).







\paragraph{Benchmark Datasets for Covariate Shift:} 
Several variants of the ImageNet dataset have been introduced to benchmark robustness against distributional shifts of models trained on the original ImageNet dataset.
\citet{hendrycks2019benchmarking} introduce two variants of the original ImageNet validation set: ImageNet-C benchmark for input corruption robustness and the ImageNet-P dataset for input perturbation robustness. 
\citet{hendrycks2019natural} present ImageNet-A which contains real-world unmodified samples that falsify state-of-the-art image classifiers. 
\citet{hendrycks2020many} present a series of benchmarks for measuring model robustness to variations on image renditions (ImageNet-R benchmark), imaging time and geographic location (StreetView benchmark), and objects size, occlusion, camera viewpoint, and zoom (DeepFashion Remixed benchmark). 
\citet{recht2019imagenet} collected ImageNet-V2 using the same data source and collection pipeline as the original ImageNet paper \cite{deng2009imagenet}.
This new benchmark leads to the observation that the prediction accuracy of even the best image classifiers are still highly sensitive to minutiae of the test set distribution and extensive hyperparameter tuning. 
Shifts \cite{malinin2021shifts} is a very recently published benchmark dataset for distributional shifts beyond the computer vision tasks.
% Taori et al.~\cite{taori2020measuring} evaluated 204 ImageNet models in 213 test conditions with different distribution shifts, only to find little to no transfer of robustness from current synthetic to natural distribution shift. 
% They suggested training on larger and more diverse datasets to be a most effective option to increase robustness, yet still being far from closing the performance gaps.
% Santurkar \textit{et al.} present Breeds~\cite{santurkar2020breeds}, a suite of subdomain shift benchmarks of varying granularity. 
% They define data subdomains as a way to evaluate how well models can generalize beyond the limited diversity of source training datasets.
% In the video domain, \citet{shankar2019image} utilize temporal consistency in video frames to construct image-level robustness benchmarks: they assembled sets of contiguous video frames that appear perceptually similar to humans, but produce inconsistent predictions for classifiers. 
% gu2019using


\paragraph{Benchmark Datasets for Label Distribution Shift:} 
Synthetic label distribution shift is commonly used for evaluation \cite{lipton2018detecting,wu2021online}: the test samples are manually sampled according to a predefined target label distribution $p_T(y)$ which is different from the source label distribution $p_S(y)$.
Recently, \cite{wu2021online} constructed a real-world label distribution shift dataset for the paper category prediction task. Specifically, the authors collected papers from 23 categories on arXiv and extracted the tf-idf vector from the abstract as the features.


\paragraph{Benchmark Datasets for OOD Detection:}
The semantically coherent OOD (SC-OOD) benchmarks \cite{yang2021semantically} are the latest ones on CIFAR10 and CIFAR100, which fixed some sever defects of previous designs.
ImageNet-O \cite{hendrycks2019natural}, containing 2000 images from 200 classes within ImageNet-22k and outside ImageNet, is a commonly used for ImageNet.
Hendrycks et al. \cite{hendrycks2019scaling} presented three large-scale and high-resolution OOD detection benchmarks for multi-class and multi-label image classification, object detection, and semantic segmentation, respectively. 
The recent ``SegmentMeIfYouCan'' benchmark \cite{chan2021segmentmeifyoucan} has two tasks: anomalous object segmentation and  road obstacle segmentation. 


\vspace{-0.5em}
\subsection{Robustness against Adversarial Attacks}
\label{sec:adversarial_attack}
Adversarial attacks add synthetic perturbations (termed as adversarial perturbations) onto the original clean sample. 
The perturbed sample, known as adversarial sample, is intended to cause wrong predictions on machine learning models, while keeping the identical semantic meaning of the clean sample. 
Different forms of adversarial perturbations have been studied on different types of data.
On image data, typical forms include the $\ell_p$ constrained additive perturbation \cite{goodfellow2014explaining}, spatial perturbation~\cite{xiao2018spatially}, and semantically meaningful perturbation~\cite{qiu2020semanticadv}. 
Beyond the image data, adversarial attacks can also be designed, such as by altering the shape of 3D surfaces \cite{xiao2019meshadv}, by replacing words with synonyms \cite{ren2019generating} or rephrasing the sentence \cite{iyyer2018adversarial} in natural language data, by applying adversarial printable 2D patches on real-world physical objects \cite{brown2017adversarial}, etc. 


\paragraph{Benchmark Datasets:} 
Robustness against adversarial attacks (also known as adversarial robustness) is usually evaluated as the empirical performance (e.g., accuracy in image classification tasks) on the adversarial samples. 
The key requirement for a faithful evaluation is that the attackers should try their best to break the model. 
There are two commonly used strategies to achieve this goal.
% This is nontrivial, since it is infeasible to search for the strongest adversarial samples. 
First, an ensemble of multiple strong and diverse adversarial attacks should be simultaneously used for evaluation. 
A typical setting for such ensemble is the AutoAttack \cite{croce2020reliable}, which consists of four state-of-the-art white-box attacks and two state-of-the-art black-box attacks. 
Another setting is used to create evaluation benchmarks of ImageNet-UA and CIFAR-10-UA \cite{kang2019testing}, which contains both $\ell_p$ constrained adversarial attacks and real-world adversarial attacks such as worst-case image fogging. 
% RobustBench \cite{croce2020robustbench} is another standardized benchmark of adversarial robustness, which as accurately as possible reflects the robustness of the considered models within a reasonable computational budget. 
% The authors evaluate model robustness against AutoAttack \cite{croce2020reliable} and also analyzed general trends in adversarial robustness and its impact on other tasks such as robustness to various distribution shifts and out-of-distribution detection. 
Second, the attacks should be carefully designed to prevent the ``gradient obfuscation'' effect \cite{athalye2018obfuscated,carlini2017adversarial}.
Since the success of traditional white-box attacks depends on accurate calculation of model gradient, they may fail if the model gradient is not easily accessible (e.g., the model has non-differential operations). 
As a result, evaluating model robustness on such attacks may provide a false sense of robustness. 
\citet{athalye2018obfuscated} proposed three enhancement for traditional white-box attacks as solutions for common causes of gradient obfuscation.
Other solutions include designing adaptive attacks for each specific defense strategy \cite{tramer2020adaptive}.
% \citet{carlini2017adversarial} and \citet{athalye2018obfuscated} emphasize on the importance of evaluation pipelines to measure defense robustness against diverse attacks. 
% For example, \citet{papernot2017practical} introduce gradient masking as a category of failed defense methods that work by trying to deny the attacker access to a useful gradient.
% On the importance of defense evaluation, \citet{carlini2017adversarial} propose three stronger threat models which can break the fake robustness achieved by gradient masking. 
% \citet{athalye2018obfuscated} propose the techniques including the Backward Pass Differentiable Approximation, Expectation Over Transformation, and reparameterization techniques to overcome the gradient masking problems. 

==> sections/3-ML-dependibility_haotao_.tex <==


% % >>> [domain shift] --> manually perturbed 
%                      --> seasonal change/locations changes 
% % - ImageNet-A and ImageNet-O: used different test source --> [domain shift]
% % - ImageNet-R:                [domain shift]
% % - ImageNet-C and ImageNet-P: [domain shift]
% - BDD-100k dataset \cite{yu2020bdd100k} covers diverse weather conditions (sunny/rainy/snowy) and different time of day (daytime/nighttime/dusk/dawn) to benchmark autonomous driving scenes. 
% % - ImageNet-9: 

% >>> [generalization error] --> 
% -            : used the same dataset
% ImageNet-v2: used the same collection pipeline --> [generalization error]


%% 1- Empirical Error:      generalization error on i.i.d test set
%% 2- Distributional Error: generalization error on (naturally shifted/perturbed test set)
%% 3- Adversarial Error:    generalization error on (adv. perturbed test set)


\section{ML Dependability}
\label{sec:error-types}

Dependability is the model's ability to minimize prediction risk on test samples. 
% Unlike code-based algorithms, the dependability of ML algorithms is bounded to the model's learning capacity and statistical assumptions under which the model is trained.
% Examples of these assumptions include the independent and identically distribution (i.i.d) relation of source and target domains. 
% % and the assumption for uniform distribution of data across all classes (i.e., class balance) \cite{domingos2012few,l2017machine}. % We don't discuss imbalanced datasets so this is removed.
% However, maintaining data distribution assumptions when deployed in the open-world is challenging and results in different types of prediction errors. 
In this section, we categorize model dependability into three different dimensions: generalization error (Sec. \ref{sec:generalization_error}), robustness against distributional shift (Sec. \ref{sec:distributional_shift}), and robustness against adversarial attacks (Sec. \ref{sec:adversarial_attack}).
% as a unified ``big picture'' to achieve dependable and robust ML models in open-world. 
Additionally, we review benchmark datasets commonly used for each type of model dependability.

\vspace{-0.5em}
\subsection{Generalization Error} \label{sec:generalization_error}
The first and foremost goal of machine learning is to minimize the \emph{generalization error}.
Given a hypothesis $h$ (e.g., a DNN with learned parameters), the generalization error (also know as the \emph{true error} and denoted as $R(h)$) is defined as the expected error of $h$ on the data distribution $\mathcal{D}$~\cite{mohri2018foundations}:
$
    R(h) = \text{Pr}_{(x,y) \sim \mathcal{D}}[h(x)\neq y] = \mathbb{E}_{(x,y) \sim \mathcal{D}}[\mathbbm{1}_{h(x)\neq y}],
$
where $(x,y)$ is a pair of data and label sampled from $\mathcal{D}$, and $\mathbbm{1}$ is the indicator function. 
The generalization error is not directly computable, since $\mathcal{D}$ is usually unknown. 
The \textit {de facto} practical solution is to learn $h$ by empirical risk minimization (ERM) on the training set $\mathbb{S}_{S}=\{(x_i,y_i)\}_{i=1}^{N_S}$ and estimate its generalization error by the \emph{empirical error} on the holdout test set $\mathbb{S}_{T}=\{(x_i,y_i)\}_{i=1}^{N_T}$. 
Formally, the empirical error $\hat{R}(h)$ is defined as the mean error on a finite set of data points $\mathbb{S} \sim \mathcal{D}^{m}$~\cite{mohri2018foundations}:
$
    \hat{R}(h) = \frac{1}{m} \sum_{i=1}^{m} \mathbbm{1}_{h(x_i)\neq y_i},
$
where $\mathbb{S} \sim \mathcal{D}^{m}$ means $\mathbb{S}=\{(x_i,y_i)\}_{i=1}^m \overset{i.i.d.}{\sim} \mathcal{D}$.
The training and test sets are all sampled from the same distribution $\mathcal{D}$ but are disjoint.
% Consider a model learned by empirical risk minimization (ERM) on training set $S=\{(x_i,y_i)\}_{i=1}^N$ i.i.d sampled from the underlying distribution $\mathcal{D}$.
% The model should not only fit $S$ by minimizing the empirical error $\mathcal{L}_\mathcal{S}(f)=\frac{1}{N}\sum_{x \in \mathcal{S}}~\mathcal{L}(x)$, but also have low generalization error on unseen data $\mathcal{L}_\mathcal{D}(f)=\mathbb{E}_{x \in \mathcal{D}} ~\mathcal{L}(x)$. 
% The generalization gap is defined as the difference between the model performance on training data and unseen data sampled from the same distribution, is a commonly used metric to evaluate model generalization ability.
% The \textit {de facto} method nowadays of probing generalization is to split the available dataset into two (or three) subsets: one for training, (one for validation), and the other for testing. The goodness of fit on the test set provides an approximation of generalization beyond training. 
Recent years have witnessed the successful application of this holdout evaluation methodology to monitoring the progress of many  ML fields, especially where large-scale labeled datasets are available. 
The generalization error can be affected by many factors, such as training set quality (e.g., imbalanced class distribution \cite{haixiang2017learning}, noisy labels \cite{bouguelia2018agreeing}), model capacity, and the training methods (e.g., using pre-training \cite{mahajan2018exploring}, regularization \cite{bansal2018can}, etc.)
% Multiple factors such as weak representation learning affect the model's generalization error which is common in open-world setups \cite{jakubovitz2019generalization}. % (e.g., model over-fitting or under-fitting on the training set)
% On the importance of generalizable representation learning, Zhang et al. \cite{Zhang2017generalization} pointed out the capacity of large DNNs is sufficient enough to memorize a small training set even in the case of random labels without any correlation between training labels and test labels. 
% On the other hand, the training set quality can greatly affect model generalization error as many assumptions such as uniform distribution of training data may not be easy to achieve in open and uncontrolled environments. 
% This is because of the large number of model parameters in the network that may exceed the number of data points in training sets, resulting in relatively small generalization error on their test set, but a high error rate on slight domain shifts within the same label space (i.e., hyper-parameter over-fitting). 
% However, representation learning gets more difficult when aiming for more complex tasks and using data with higher dimensionality. 


\paragraph{Benchmark Datasets:} 
Model generalization is commonly evaluated on a separate test set provided for the dataset.
However, recent research has found limitations of such evaluation strategy. 
For example, \citet{wang2020going} showed that the fixed ImageNet \cite{deng2009imagenet}  test set is not sufficient to reliably evaluate the generalization ability of state-of-the-art image classifiers, due to the insufficiency in representing the rich visual open-world.
% Other efforts have been made to collect new samples to improve test sets for image classification tasks. % as complements for the original ImageNet test set. 
\citet{tsipras2020imagenet} observed that noisy data collection pipeline can lead to a systematic misalignment between the training sets and the real-world tasks. % a brittleness that puts claims about human-level performance into context.



\vspace{-0.5em}
\subsection{Robustness against Distributional Shifts} 
\label{sec:distributional_shift}
When measuring generalization error, we assume the source training set $\mathbb{S}_S$ and the target test set $\mathbb{S}_T$ are from the same data distribution. 
However, this assumption is frequently violated in real world applications. In other words, we will have $p_S(x,y) \neq p_T(x,y)$ where $p_S(x,y)$ and $p_T(x,y)$ are the joint probability density distributions of data $x$ and label $y$ on the training and test distributions, respectively.
Such mismatch between training and test data distribution is known as \textit{dataset shift}~\cite{quinonero2009dataset} (also termed as \textit{distributional shift} or \textit{domain shift} in literature).
In this paragraph, we describe two most common distributional shifts and their benchmark datasets. 
\textit{Covariate shift} means that the training and test distributions of the input covariate $x$ are different (i.e., $p_S(x) \neq p_T(x)$), while the labeling function remains the same (i.e., $p_S(y|x) = p_T(y|x)$). 
Covariate shift may occur due to natural perturbations (e.g., weather and lighting changes), data changes over time (e.g., seasonal variations of data), and even more subtle digital corruptions on images (e.g., JPEG compression and low saturation). 
\textit{Label distribution shift} (also know as \textit{prior probability shift}) is the scenario when the marginal distributions of $y$ changes while the class-conditional distribution remains the same. Formally, it is defined as $p_S(y) \neq p_T(y), p_S(x|y) = p_T(x|y)$.  
Prior probability shift is typically concerned in applications where the label $y$ is the casual variable (e.g., pneumonia) for the observed feature $x$ (e.g., chest X-ray) \cite{lipton2018detecting}. For example, if we trained a pneumonia predictor using the chest X-ray data collected in summer (when $p(y)$ is low), we may still require it to be accurate on patients visiting in winter (when $p(y)$ is high).
A special case for label distributional shift is long-tailed recognition \cite{van2017devil}, where the training set is long-tail distributed (i.e., $p_S(y)$ follows a long-tailed distribution) while the test set is balanced (i.e., $p_T(y)$ roughly follows a uniform distribution).

% Domain shift (also known as distribution shift and dataset shift) describes variations in the target data distribution ($D_{target}$) in comparison to the source training distribution ($D_{train}$). 
% Distributional error is the misprediction of target samples due to inconsistency between source and target distributions and hence reduces the \textit{Operational Performance} compared to the test set (on $D_{test}$) performance.
% Specifically, distributional error reduces the operational performance compared to the training set performance (on $D_{test}$) by breaking the i.i.d assumption between source and target data. 
% In this regard, robust training techniques (e.g., transfer learning, domain generalization) are necessary elements in training ML models for open-world applications in which target samples are captured from uncontrolled and constantly changing environments (see Section \ref{sec:RT} for details).

% Common examples of domain shift include non-semantic distribution changes due to input perturbations (e.g., natural perturbations due to weather and lighting changes), data changes over time (e.g., seasonal variations of data), and even more substantial texture and breed variations. % geographic locations.
% In general, the problem of ``domain shift" is rooted in the fundamental contradiction between the enormous size and high dimensionality of natural image manifold, and the limited scale of affordable testing (i.e., human labeling, or verifying predicted labels, which is expensive and time consuming).
% Model comparison based on a limited number of samples assumes that they are \textit{sufficiently representative} of the whole population, an assumption that has been proven to be doubtful in computer vision tasks. 
% On studies to measure the distributional error, different work shows that using a fixed test set are insufficiently representative of the whole target distribution. 
% For instance, Recht et al. \cite{recht2018cifar,recht2019imagenet} found that a minute natural distribution shift leads to a large drop in accuracy for a broad range of image classifiers on both CIFAR-10~\cite{krizhevsky2009learning} and ImageNet. %  suggesting that the current test sets may be far from sufficient to represent hard natural images encountered in the real world. 


% Beyond generalization to reasonably foreseeable domain shifts, Out-of-Distribution (OOD) or outlier samples are referred to undesirable test-time samples with disjoint label space and high semantic discrepancy. 
Beyond the above reasonably foreseeable domain shifts, a model may also encounter out-of-distribution (OOD) test samples with semantic contents unseen in the training distribution. 
For example, for a classifier trained on hand-written digit images, a Roman character is an OOD test sample (while a printed digit is a test sample with domain gap).
\textit{OOD detection} \cite{hendrycks2016baseline} is the approach to detect such OOD samples, whose predictions will be rejected (see Section \ref{sec:ood-detection} for details).







\paragraph{Benchmark Datasets for Covariate Shift:} 
Several variants of the ImageNet dataset have been introduced to benchmark robustness against distributional shifts of models trained on the original ImageNet dataset.
\citet{hendrycks2019benchmarking} introduce two variants of the original ImageNet validation set: ImageNet-C benchmark for input corruption robustness and the ImageNet-P dataset for input perturbation robustness. 
\citet{hendrycks2019natural} present ImageNet-A which contains real-world unmodified samples that falsify state-of-the-art image classifiers. 
\citet{hendrycks2020many} present a series of benchmarks for measuring model robustness to variations on image renditions (ImageNet-R benchmark), imaging time and geographic location (StreetView benchmark), and objects size, occlusion, camera viewpoint, and zoom (DeepFashion Remixed benchmark). 
\citet{recht2019imagenet} collected ImageNet-V2 using the same data source and collection pipeline as the original ImageNet paper \cite{deng2009imagenet}.
This new benchmark leads to the observation that the prediction accuracy of even the best image classifiers are still highly sensitive to minutiae of the test set distribution and extensive hyperparameter tuning. 
Shifts \cite{malinin2021shifts} is a very recently published benchmark dataset for distributional shifts beyond the computer vision tasks.
% Taori et al.~\cite{taori2020measuring} evaluated 204 ImageNet models in 213 test conditions with different distribution shifts, only to find little to no transfer of robustness from current synthetic to natural distribution shift. 
% They suggested training on larger and more diverse datasets to be a most effective option to increase robustness, yet still being far from closing the performance gaps.
% Santurkar \textit{et al.} present Breeds~\cite{santurkar2020breeds}, a suite of subdomain shift benchmarks of varying granularity. 
% They define data subdomains as a way to evaluate how well models can generalize beyond the limited diversity of source training datasets.
% In the video domain, \citet{shankar2019image} utilize temporal consistency in video frames to construct image-level robustness benchmarks: they assembled sets of contiguous video frames that appear perceptually similar to humans, but produce inconsistent predictions for classifiers. 
% gu2019using


\paragraph{Benchmark Datasets for Label Distribution Shift:} 
Synthetic label distribution shift is commonly used for evaluation \cite{lipton2018detecting,wu2021online}: the test samples are manually sampled according to a predefined target label distribution $p_T(y)$ which is different from the source label distribution $p_S(y)$.
Recently, \cite{wu2021online} constructed a real-world label distribution shift dataset for the paper category prediction task. Specifically, the authors collected papers from 23 categories on arXiv and extracted the tf-idf vector from the abstract as the features.


\paragraph{Benchmark Datasets for OOD Detection:}
The semantically coherent OOD (SC-OOD) benchmarks \cite{yang2021semantically} are the latest ones on CIFAR10 and CIFAR100, which fixed some sever defects of previous designs.
ImageNet-O \cite{hendrycks2019natural}, containing 2000 images from 200 classes within ImageNet-22k and outside ImageNet, is a commonly used for ImageNet.
Hendrycks et al. \cite{hendrycks2019scaling} presented three large-scale and high-resolution OOD detection benchmarks for multi-class and multi-label image classification, object detection, and semantic segmentation, respectively. 
The recent ``SegmentMeIfYouCan'' benchmark \cite{chan2021segmentmeifyoucan} has two tasks: anomalous object segmentation and  road obstacle segmentation. 


\vspace{-0.5em}
\subsection{Robustness against Adversarial Attacks}
\label{sec:adversarial_attack}
Adversarial attacks add synthetic perturbations (termed as adversarial perturbations) onto the original clean sample. 
The perturbed sample, known as adversarial sample, is intended to cause wrong predictions on machine learning models, while keeping the identical semantic meaning of the clean sample. 
Different forms of adversarial perturbations have been studied on different types of data.
On image data, typical forms include the $\ell_p$ constrained additive perturbation \cite{goodfellow2014explaining}, spatial perturbation~\cite{xiao2018spatially}, and semantically meaningful perturbation~\cite{qiu2020semanticadv}. 
Beyond the image data, adversarial attacks can also be designed, such as by altering the shape of 3D surfaces \cite{xiao2019meshadv}, by replacing words with synonyms \cite{ren2019generating} or rephrasing the sentence \cite{iyyer2018adversarial} in natural language data, by applying adversarial printable 2D patches on real-world physical objects \cite{brown2017adversarial}, etc. 


\paragraph{Benchmark Datasets:} 
Robustness against adversarial attacks (also known as adversarial robustness) is usually evaluated as the empirical performance (e.g., accuracy in image classification tasks) on the adversarial samples. 
The key requirement for a faithful evaluation is that the attackers should try their best to break the model. 
There are two commonly used strategies to achieve this goal.
% This is nontrivial, since it is infeasible to search for the strongest adversarial samples. 
First, an ensemble of multiple strong and diverse adversarial attacks should be simultaneously used for evaluation. 
A typical setting for such ensemble is the AutoAttack \cite{croce2020reliable}, which consists of four state-of-the-art white-box attacks and two state-of-the-art black-box attacks. 
Another setting is used to create evaluation benchmarks of ImageNet-UA and CIFAR-10-UA \cite{kang2019testing}, which contains both $\ell_p$ constrained adversarial attacks and real-world adversarial attacks such as worst-case image fogging. 
% RobustBench \cite{croce2020robustbench} is another standardized benchmark of adversarial robustness, which as accurately as possible reflects the robustness of the considered models within a reasonable computational budget. 
% The authors evaluate model robustness against AutoAttack \cite{croce2020reliable} and also analyzed general trends in adversarial robustness and its impact on other tasks such as robustness to various distribution shifts and out-of-distribution detection. 
Second, the attacks should be carefully designed to prevent the ``gradient obfuscation'' effect \cite{athalye2018obfuscated,carlini2017adversarial}.
Since the success of traditional white-box attacks depends on accurate calculation of model gradient, they may fail if the model gradient is not easily accessible (e.g., the model has non-differential operations). 
As a result, evaluating model robustness on such attacks may provide a false sense of robustness. 
\citet{athalye2018obfuscated} proposed three enhancement for traditional white-box attacks as solutions for common causes of gradient obfuscation.
Other solutions include designing adaptive attacks for each specific defense strategy \cite{tramer2020adaptive}.
% \citet{carlini2017adversarial} and \citet{athalye2018obfuscated} emphasize on the importance of evaluation pipelines to measure defense robustness against diverse attacks. 
% For example, \citet{papernot2017practical} introduce gradient masking as a category of failed defense methods that work by trying to deny the attacker access to a useful gradient.
% On the importance of defense evaluation, \citet{carlini2017adversarial} propose three stronger threat models which can break the fake robustness achieved by gradient masking. 
% \citet{athalye2018obfuscated} propose the techniques including the Backward Pass Differentiable Approximation, Expectation Over Transformation, and reparameterization techniques to overcome the gradient masking problems. 

==> sections/9-conclusion.tex <==
\vspace{-0.5em}
\section{Conclusion}

We proposed a categorization for broad range of ML techniques that support algorithmic safety for open-world deployment of ML based software.
Our organization of ML techniques is supported by a thorough reviewing of key papers in each branch. 
At the end, we identified open problems and research directions that can benefit from research community. 
We hope our categorization and review helps in building new ML safety guidelines and development frameworks for safety-critical applications. 


% \begin{acknowledgements}
% Acknowledgements is removed for \textit{Anonymous Review}.
% \end{acknowledgements}


==> sections/notepad.tex <==

\subsubsection*{T3.1 Well-Established ML Solutions}
% S1: Inherently Safe Design
\textbf{Visualization Tools, Global and Local Explanations: }
\newline

\textbf{Semi-Formal Verification, Formal Testing, and End-to-End Testing: } Recent advancements in scientific simulation \cite{lavin2021simulation} and 3D environment rendering (e.g., \cite{NVDriveSim,Shah2018AirSim}) have introduced promising solutions for end-to-end testing and semi-formal verification of ML systems. % koren2021finding
However, it is challenging to mitigate the gap between simulation and real-world situations, causing questionable transfer of simulated verification and testing results. Recent work starts exploring how formal simulation aid in designing real-world tests \cite{fremont2020formal}.
\newline

% S2: Robust and Dependable Machine Learning
\textbf{Model Capacity, Structure and Operations: } Research and industrial trends show...
\newline

\textbf{Transfer Learning and Pretraining: } Early advancement in deep learning led to benefits of transfer learning and pretraining for machine learning models. 
Another less explored direction for ML robustness is to benefit from multi-domain and multi-source training data for improved representation learning. 
The rich contexts captured from sensor sets with diverse orientations and data modality can significantly improve prediction robustness compared to a single input source (e.g., single camera). % against distribution shifts and artifacts.
Self-checking based on temporal and semantic coherence of data could also be exploited to enhancing robustness and performance in practical applications such as autonomous vehicles. 
\newline


\textbf{Robust Training, Training Regularization: } 
Despite advances in studying natural corruptions, distributional shift and adversarial robustness, respectively, there lacks systematic efforts to tackle robustness limitations in a unified framework to cover the ``in-between" cases within this spectrum. 
Historically, the study of one robustness type does not always translate to benefiting other types. 
The recent paper \cite{dreossi2019formalization} formalized various types of robustness that the research communities have considered in the literature, yielding a unifying quantitative-Boolean formulation of robustness. 
To date, most robustness work has focused on model invariances to small perturbations.  
However, alternate specifications for properties directly relevant in real-world can offer more favorable research opportunities. 
One example of practical relevance is to perturb in the semantic feature spaces: modeling the underlying semantic context in which ML systems operate can be crucial to scale up analysis and also provide more meaningful task-oriented results \cite{robey2020model}. 
\newline

\textbf{Active Learning, Hardness Weighted Sampling, Data Cleansing, and Augmentation:}

% S3: Uncertainty Awareness and Self-Assessment
\textbf{Uncertainty Calibration and Estimation: }
There are profound demands to research and develop new ML techniques for system self-assessment of task confidence or skill proficiency in a dynamic environment where the input distribution or the task goal may vary.  
Although current efforts mostly arise from Bayesian statistics and data-driven calibration, domain knowledge is a crucial component to benefit from in open-world applications.
For example, incorporating prior knowledge from physical phenomena like sensor noise and lighting conditions can be cast into information theoretical forms for robust uncertainty estimation \cite{loquercio2020general}.  % ,pires2020towards
Another practical and understudy uncertainty-aware design proposed in \cite{mcallister2017concrete} is to use prediction uncertainty together with the prediction itself to impact downstream decision-making and planning tasks in the system and in cases request for human assistant.


\subsubsection*{T3.2 Emerging ML Solutions}
% S1: Inherently Safe Design

% S2: Robust and Dependable Machine Learning
Adversarial Training and Adversarial Guard\\
Domain Randomization\\
Robust Representation Learning\\
Multi-source Training

% S3: Uncertainty Awareness and Self-Assessment
Adversarial Attack and Out-of-distribution Detection


\subsubsection*{T3.3 Future ML Solutions}
% S1: Inherently Safe Design
Model Specification\\
Formal Verification

% S2: Robust and Dependable Machine Learning
language-Image Models\\
Knowledge-based and ...
% S3: Uncertainty Awareness and Self-Assessment




==> tables/table_old_.tex <==
% Link to tables: https://docs.google.com/spreadsheets/d/1Pwk9q_53aGGFcegfdIwpQPPdddBJpPdNPYO1gqs2800/edit#gid=0


\begin{table*}[]
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\centering
\caption{Comparison between safety standards gaps for ML components and fundamental safety limitations of ML algorithms. \TODO{better caption}}
\label{tab:my-table}
\begin{tabular}{ccc}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Gaps in Safety Standards \\ for ML Components\end{tabular}} & \textbf{Fundamental ML Safety Limitations} & \textbf{\begin{tabular}[c]{@{}c@{}}Machine Learning and \\ Software Safety Research\end{tabular}} \\ \hline
\multirow{2}{*}{Code Review} & Not code-based & ([ref]) \\ \cline{2-3} 
 & Not specifiable & ([ref]) \\ \hline
Software Safety Requirements Specification & Data-driven model training & ([ref]) \\ \hline
Software Architectural Design & Not code-based & ([ref]) \\ \hline
Software Unit Design & Non-converx optimization & ([ref]) \\ \hline
\multirow{2}{*}{Unit, Integration and System Testing} & Not Verifiable & ([ref]) \\
 & Non-deterministic & ([ref]) \\ \hline
Traceability & Not Transparent ([ref]) & ([ref]) \\ \hline
\end{tabular}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \centering
% \caption{Algorithm dependability methods to complement functional safety and SOTIF safety methods for machine learning safety.}
% \label{tab:my-table}
% \begin{tabular}{ccc}
% \hline
% \begin{tabular}[c]{@{}c@{}}Gaps in Safety Standards \\ for ML Components\end{tabular} & Fundamental ML Safety Limitations & Machine Learning Dependability Method \\ \hline
% \multirow{2}{*}{Code Review} & Not specifiable & [ref] ...[ref] \\ \cline{2-3} 
%  & Non-deterministic & ...[ref] ...[ref] \\ \hline
% Software Safety Requirements Specification & xxxx & yyy: [ref] xxx [ref] \\ \hline 
% Software Architectural Design & xxxx & yyy: [ref] xxx [ref] \\ \hline
% Software Unit Design & Non-converx optimization & Dataset analysis: [ref] Regularization [ref] \\ \hline
% Unit, Integration and System Testing & Not Verifiable & Uncertainty Extraction: XX [ref] \\ \hline
% \multicolumn{1}{|c|}{Traceability} & Not Transparent & ... [ref] \\ \hline
% \end{tabular}
% \end{table*}



% \begin{table*}[]
% \centering
% \caption{Algorithm dependability methods to complement functional safety and SOTIF safety methods for machine learning safety.}
% \label{tab:my-table}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}cccc@{}}
% \toprule
%  & ISO Software Safety Clause/Term & DNN Safety Limitations & Machine Learning Dependability Method \\ \midrule
% \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\rotatebox{90}{Functional Safety} \end{tabular}} \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\rotatebox{90}{(ISO 26262-6)} \end{tabular}} 
% & \multirow{2}{*}{Software Requirements Specification} & Not specifiable & Run-time Outlier Detection: ...[ref] ...[ref] \\ \cmidrule(l){3-4} 
%  &  & Non-deterministic & ...[ref] ...[ref] \\ \cmidrule(l){2-4} 
%  & Software Unit Design & Non-converx optimization & Dataset analysis: [ref] Regularization: ref] \\ \cmidrule(l){2-4} 
%  & \multirow{2}{*}{Software Unit Verification} & Not Verifiable & Uncertainty Extraction: XX [ref] \\ \cmidrule(l){3-4} 
%  &  & Not Transparent & ... [ref] \\ \midrule
% \multirow{3}{*}{\rotatebox{90}{SOTIF}} & Functional modifications to reduce SOTIF Related Risks & Robustness & ...[ref] [ref] \\ \cmidrule(l){2-4} 
%  & Verification for known-unface Scenarios &  & ...[ref] [ref] \\ \cmidrule(l){2-4} 
%  & Validation of Unknown-Unsafe Scenarios &  & ... [ref] [ref] \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}
